A Survey of Scheduling Algorithms for the Time-Aware Shaper in Time-Sensitive Networking (TSN)

Time-Sensitive Networking (TSN) is an enhancement of Ethernet which provides various mechanisms for real-time communication. Time-triggered (TT) traffic represents periodic data streams with strict real-time requirements. Amongst others, TSN supports scheduled transmission of TT streams, i.e., the transmission of their frames by end stations is coordinated in such a way that none or very little queuing delay occurs in intermediate nodes. TSN supports multiple priority queues per egress port. The TAS uses so-called gates to explicitly allow and block these queues for transmission on a short periodic timescale. The TAS is utilized to protect scheduled traffic from other traffic to minimize its queuing delay. In this work, we consider scheduling in TSN which comprises the computation of periodic transmission instants at end stations and the periodic opening and closing of queue gates. In this paper, we first give a brief overview of TSN features and standards. We state the TSN scheduling problem and explain common extensions which also include optimization problems. We review scheduling and optimization methods that have been used in this context. Then, the contribution of currently available research work is surveyed. We extract and compile optimization objectives, solved problem instances, and evaluation results. Research domains are identified, and specific contributions are analyzed. Finally, we discuss potential research directions and open problems.

==> chapters/03_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
To the best of our knowledge, no other published literature overview is concerned with scheduling algorithms for TSN. 
In fact, there is no survey about scheduling for time-triggered flows in time-sensitive Ethernet networks, regardless of the used standard.
However, there are surveys which intersect with the content of this work.

Minaeva et al. \cite{MiHa21} give a literature summary for scheduling time-triggered real time systems.
They highlight research works from 1968 -- 2020.
As opposed to this work, they not only consider scheduling of flows in networks, but all systems with periodic schedules.
Highly influential works for TNS scheduling algorithms in the literature are mentioned, e.g., \cite{St10} and \cite{ScDa17}.
Out of 126 references, only 6 of them intersect with this work.

Deng et al. \cite{DeXe22} review a wide range of topics about AVB and TSN from the literature of 2007 -- 2021. 
Besides scheduling approaches, they also give an overview of reliability and security modeling, and delay analysis in the mentioned areas.
As a wider range of topics is covered, only a small part of the survey is concerned with scheduling.
This part is rather superficial, summarizes only 15 works, and is mostly in tabular form.
Evaluation findings, scalability, and detailed descriptions of the proposed algorithms are omitted.
All in all, 17 out of the 128 discussed works intersect with this survey.

Seol et al. \cite{SeHy21} review TSN as a whole.
The authors cover publications of the years 2014 -- 2020.
An overview of active research directions is given, including computing routings and schedules in TSN.
Not only the literature about scheduling for 802.1Qbv is summarized, but also work concerned with other queuing mechanisms, hardware, and simulator frameworks.
Therefore, like in \cite{DeXe22}, only a small fraction of the literature about scheduling for TAS-based queuing in TSN is surveyed. 
They cover 207 research works, of which 29 are included in this literature overview.
The works in intersection with this survey are merely mentioned, and the authors do not elaborate on their content. 

==> chapters/04_overview.tex <==
\section{Literature Overview}
\label{sec:literature_overview}
In the following sections, we give a overview of research work about \ac{TSN} scheduling algorithms.
\SL{We categorize the reviewed literature by the applied optimization technique and describe their core properties.}
%First, we present a summary of solution approaches and evaluations presented in the literature.
Then, we first categorize research work based on the optimization methods used and second on the objectives of the scheduling algorithms.

%\subsection{Solution Approaches}
%In the following, we classify the body of research literature by solution approach and summarize the purpose of the various algorithms.
\subsection{\acf{ILP}}
\SL{No-wait schedules assume no queuing delay and enforce that a frame is immediately forwarded when it enters a queue.}
%No-wait schedules assume that the only delay a bridge imposes to a frame is processing delay, so frames are immediately forwarded when they enter a queue.
Duerr et al. \cite{DuNa16} propose an \ac{ILP} and a Tabu Search algorithm to compute no-wait schedules of flows. 
They model the problem with the job-shop scheduling, a widely used modelling framework in the scheduling literature.
They also propose a compression algorithm as post-processing for schedules, which aims to reduce the number of GCL entries needed to implement the schedule. 
In later works, Falk et al. \cite{FaDu18} extend the \ac{ILP} from \cite{DuNa16} to simultaneously compute routing and scheduling of \ac{TT} flows.
They analyze the scalability of the joint routing and scheduling problems using \acp{ILP}.
Another independently developed \ac{ILP} model, which addresses the problem of joint scheduling and routing, is presented in \cite{ScDa17}.
Although it is not exclusively for \ac{TSN}, the authors state it is applicable for such networks.
An \ac{ILP} approach for fault tolerant joint scheduling and routing can be found in \cite{AtBa20}.
Atallah et al. \cite{AtBa20} propose an iterative scheme, where groups of flows are scheduled one after another. 
The partitioning of flows is done by introducing a conflict metric and computing a weighted cut of the conflict graph.
The authors of \cite{PoRa16} give an \ac{ILP} to compute schedules for \ac{TT} flows and additionally present a \ac{GRASP} heuristic to schedule \ac{AVB} flows. 
They compute routing and scheduling of \ac{AVB} flows simultaneously with the optimal scheduling for \ac{TT} flows as input parameters and compare their results with \cite{CrOl16}.  
Recent work from Syed et al. \cite{SyAy20} deals with in-vehicle joint scheduling and routing. 
They present an \ac{ILP} model for static flows which takes load balancing into account and aims for schedules which are suitable for dynamic adding of flows.
The authors of \cite{PoRo18} present an ILP which maximizes the distances between frames, in order to increase repairability of schedules.


\subsection{\acf{SMT}}
Craciunas et al. \cite{CrOl16} construct a \ac{SMT} modelling to schedule \ac{TT} flows.
They define flow isolation and frame isolation as properties of a schedule to prevent some sources of non-determinism.
Frame isolation forbids that frames of different flows are in a queue at the same time.
Flow isolation forbids interleaving of frames of different flows in the same queue entirely, so the first frame of a queue can only enter a queue if the last frame of the preceding flow has left it. 
They present models to compute schedules with either flow or frame isolation.
The same authors also introduce in \cite{StCr18} a formal framework for \ac{TSN} schedule verification and demonstrate the scheduling constraints with a \ac{SMT} model. 
They propose to use this framework as starting point for standardization of \ac{TSN} scheduling mechanisms. 
Another \ac{SMT} approach is presented by \cite{JiXi20}. 
Jin et al. develop an \ac{SMT} model to schedule \ac{TSN} flows with a fixed number of gate-openings, as real \ac{TSN} switches only have a limited number of \ac{GCL} entries.
As their \ac{SMT} model cannot be solved globally in reasonable time, they use an iterative scheme to schedule small groups of flows separately. 
Jin et al. also propose an \ac{SMT} model for joint message fragmentation and scheduling of \ac{TT} flows in \cite{JiXi19}.
Due to performance reasons of solving the model, they also give heuristics for message fragmentation and scheduling.
The authors of \cite{FaKu17} do not only use an \ac{SMT} solver to compute \ac{TSN} schedules, but also to analyze conflicting sets of flows with the unsatisfiable core returned by the \ac{SMT} solver. 
Houtan et al. \cite{HoAs21} compare schedules computed with various objectives for the same \ac{SMT} model with respect to \ac{QoS} of \ac{BE} traffic.
Another \ac{SMT} model which takes additional requirements into account is presented in \cite{ZhSa21}.
Zhou et al. allow the definition of reliability constraints regarding transmission fault probability in their model.
Mahfouzi et al. \cite{MaAm21} propose a \ac{SMT} model for joint scheduling and routing.
They suggest search space reductions with k-shortest paths to increase the performance of routing and scheduling.

\subsection{Other Exact Approaches}
All exact algorithms, which are not based on \ac{ILP} and \ac{SMT} models considers the joint routing and scheduling problem.
Falk et al. propose a joint routing and scheduling algorithm in \cite{FaDu20}, which is not based on constraints of flow transmissions.
Their approach constructs a conflict graph, where each vertex represents a scheduling configuration for a single flows. 
This reduces the scheduling problem to finding an independent set in this graph.
Gavrilut et al. \cite{GaZa17} also give multiple algorithms to compute scheduling and routing of \ac{TT} flows simultaneously. 
In contrast to \cite{FaDu18} these algorithms additionally synthesize the topology with minimized costs.  
They present a problem-specific heuristic, a \ac{GRASP} heuristic and a \ac{CP} approach and compare them to each other regarding solving time and solution quality.
The authors of \cite{RePo20} give a \ac{CP} modelling for joint computing of scheduling and routing, which also takes security and reliability considerations into account. 
Redundant paths are routed where needed. 
Smirnov et al. \cite{SmGl17} present a \ac{PBO} model for joint routing and scheduling. 

\subsection{Heuristic Approaches}
Hellmanns et al. \cite{HeGl20} base their work on the Tabu Search algorithm of \cite{DuNa16}. 
They evaluate it for a hierarchical network which consists of multiple rings on different layers. 
They propose to schedule the ring networks on the lowest level one after another and simulate the flows between different rings thereafter.
Raagaard et al. \cite{RaPo17} propose an approach for online scheduling of new \ac{TT} flows regarding an existing schedule.
They use a heuristic with as-soon-as-possible scheduling and queue reassignments.
Following their work in \cite{SyAy20}, Syed et al. present multiple heuristics for dynamic scheduling of new flows in an existing schedule \cite{SyAy21}. 
Various incremental algorithms to schedule \ac{TSN} flows without wasting to much bandwidth for guard bands are presented by Alnajim et al. \cite{AlSa19}.
The authors of \cite{ReZh20} present a heuristic to schedule flows without isolation constraints.
They change the transmission windows of egress queues until  all flows meet their deadline.
In contrast to earlier approaches with queuing \cite{CrOl16} \cite{OlCr18}, they drop frame and flow isolation constraints by performing worst-case end-to-end latency analysis.
Yan et al. \cite{YaQu20} show a heuristic time tabling algorithm, which uses problem specific knowledge and is based on Tabu Search.
They also present a naive algorithm and modifications of their approach, which are based on Simulated Annealing or Greedy strategies instead of Tabu Search.
The authors of \cite{WaCh20} propose a completely different approach with ant colony optimization. 
They give the fundamental building blocks of such an algorithm and demonstrate that it can be suitable for \ac{TSN} scheduling, but also note that further investigation of other problems is needed. 
Another algorithm inspired by biology is presented by Pahlevan et al. \cite{PaOb18}.
They construct a genetic algorithm for joint routing and scheduling, which also comprises advanced features like multicast flows and dependencies of flows.
In later work, Pahlevan et al. \cite{PaTa19} give two other heuristics for the same purpose. 
Gavrilut et al. \cite{GaPo18} describe how a \ac{GRASP} heuristic for joint scheduling of \ac{TT} and \ac{AVB} flows could be constructed and propose different objective functions for such a heuristic.  
The authors of \cite{PoRo18} present a repair algorithm for schedules in the case of link failures in time triggered networks.
They further analyze which properties of schedules contribute to repairability.

Table \ref{tab:approaches} compiles the solution approaches used in the literature.
Papers are listed in multiple categories if they give multiple algorithms.
The most often technique used is \ac{SMT} solving.
The numbers of exact and heuristic scheduling algorithms in the literature is roughly the same. 
\begin{table}[ht]
    \centering
    \begin{tabular}{|M{2cm}|M{5.5cm}|}
    \hline
        Method & Research work \\\hline\hline
        \ac{ILP} & Duerr et al. \cite{DuNa16}, Pop et al. \cite{PoRa16}, Schweissguth et al. \cite{ScDa17}, Falk et al. \cite{FaDu18}, Pozo et al. \cite{PoRo18}, Atallah et al. \cite{AtBa20}, Syed et al. \cite{SyAy20} \\\hline
        \ac{SMT} & Pop et al. \cite{PoRa16}, Craciunas et al. \cite{CrOl16}, Farzaneh et al. \cite{FaKu17}, Oliver et al. \cite{OlCr18}, Steiner et al. \cite{StCr18}, Jin et al. \cite{JiXi19} \cite{JiXi20}, Houtan et al. \cite{HoAs21}, Zhou et al. \cite{ZhSa21}, Mahfouzi et al. \cite{MaAm21} \\\hline
        \ac{CP} & Gavrilut et al. \cite{GaZa17}, Reusch et al. \cite{RePo20} \\\hline
        \ac{PBO} & Smirnov et al. \cite{SmGl17} \\\hline\hline
        \ac{GRASP} & Pop et al. \cite{PoRa16}, Gavrilut et al. \cite{GaZa17}  \cite{GaPo18} \\\hline
        Tabu Search & Duerr et al. \cite{DuNa16}, Hellmanns et al. \cite{HeGl20}, Yan et al. \cite{YaQu20} \\\hline
        Genetic Algorithm & Pahlevan et al. \cite{PaOb18} \cite{PaTa19}, Wang et al. \cite{WaCh20} \\\hline
        Problem Specific Heuristic & Raagaard et al. \cite{RaPo17}, Alnajim et al. \cite{AlSa19}, Falk et al. \cite{FaDu20}, Jin et al. \cite{JiXi20}, Reusch et al. \cite{ReZh20}, Syed et al. \cite{SyAy21} \\
         \hline
    \end{tabular}
    \caption{Categorization of research work based on solution approach.}
    \label{tab:approaches}
\end{table}

\subsection{Scheduling Objective}
% TODO Eileitender Text für subsection schreiben
Although all scheduling algorithms presented in this paper schedule the transmission of \ac{TT} flows, the various approaches differ in the definition of what a good schedule is.
Many research works have no scheduling objective and just try to find some schedule which fulfills all constraints, e.g. \cite{FaDu18}, \cite{RaPo17}, and \cite{FaDu20}.
Minimizing the flowspan, i.e. the time the last \ac{TT} flow reaches its destination, is a common objective when finding an optimal flow is desired.
Examples for such algorithms include \cite{DuNa16} and \cite{HeGl20}.
A related but different objective is the minimization of end-to-end delays of \ac{TT} flows, which is pursued by Schweissguth et al. \cite{ScDa17}.
Research work which considers isolation constraints for queuing often tries to minimize the number of queues reserved for \ac{TT} flows per egress port, as they introduce spatial isolation of flows by assigning them to different queues.
Such work includes \cite{CrOl16}, \cite{PoRa16}, and \cite{GaPo18}.
The minimization of \ac{GCL} entries is considered by \cite{JiXi20}, which is reasonable as the number of entries is limited in real hardware.
Reducing it also reduces the number of guard bands, which benefits \ac{BE} traffic.
Minimization of per flow jitter is pursued by \cite{OlCr18}. 
For joint scheduling of \ac{TT} and \ac{AVB} flows, Gavrilut et al. \cite{GaPo18} \cite{GaZh18} minimize the tardiness of \ac{AVB} flows, as their deadlines are not strict and the miss of a \ac{TT} flows deadline is unacceptable anyway.
Gavrilut et al. \cite{GaZa17} minimize multiple objectives, weighted by constant factors.
The first objective is the tardiness of \ac{TT} flows to guide their \ac{GRASP} heuristic to solutions with no deadline misses.
The second is topology costs, as their approach also synthesizes the topology for scheduling and routing.
The joint routing of \cite{WaCh20} minimize the number of links in the routing.
The authors of \cite{ReZh20} minimize the occupation percentage of egress ports, i.e. the percentage of a hyperperiod for which no transmission window for \ac{TT} traffic is active.
The rational of this is that low occupation corresponds to long and frequent time intervals for lower priority traffic.
The algorithm of Yan et al. \cite{YaQu20} has a maximization objective.
There heuristic tries to schedule as many flows as possible.
Syed et al. \cite{SyAy20} use a modelling specific objective which is related to load balancing of ports in a in-vehicle architecture with one central processing unit.
Pozo et al. \cite{PoRo18} maximize the idle times of links and frames, as such schedules are easier to repair upon link failure.
The work in \cite{HoAs21} focuses on different objective functions to increase the \ac{QoS} of \ac{BE} traffic.
They propose minimization and maximization of frame offsets, hoping that grouping frames together increases the \ac{QoS}. 
Additionally, they also suggest two objectives which maximize the slack between consecutive frames on a link for higher schedule porosity.
Reusch et al. \cite{RePo20} minimize ...
The authors of \cite{JiXi19} minimize the number of packets, as they propose a joint approach for scheduling and message fragmentation.
Table \ref{tab:objectives} compiles the objectives pursued in the literature.
\begin{table}[ht]
    \centering
    \begin{tabular}{|M{3.5cm}|M{4.3cm}|}
    \hline
        Objective & Research work \\\hline\hline
        No objective & Farzaneh et al. \cite{FaKu17}, Raagaard et al. \cite{RaPo17} Falk et al. \cite{FaDu18}, Steiner et al. \cite{StCr18}, Alnajim et al. \cite{AlSa19}, Falk et al. \cite{FaDu20}, Atallah et al. \cite{AtBa20}, Zhou et al. \cite{ZhSa21}, Syed et al. \cite{SyAy21}, Mahfouzi et al. \cite{MaAm21} \\\hline
        Minimize the flowspan & Dürr et al. \cite{DuNa16}, Pahlevan et al. \cite{PaOb18} \cite{PaTa19}, Hellmanns et al. \cite{HeGl20}, Houtan et al. \cite{HoAs21} \\\hline
        Minimize the latencies of the \ac{TT} flows & Schweissguth et al. \cite{ScDa17} \\\hline
        Minimize the sum of \ac{TT} queues per egress port  & Craciunas et al. \cite{CrOl16}, Pop et al. \cite{PoRa16}, Gavrilut et al. \cite{GaPo18} \\\hline
        Minimize  GCL entries & Jin et al. \cite{JiXi20} \\\hline
        Minimize the sum of per flow jitters & Oliver et al. \cite{OlCr18} \\\hline
        Minimize the sum of tardiness of \ac{AVB} flows & Gavrilut et al. \cite{GaPo18} \cite{GaZh18} \\\hline
        Other & Gavrilut et al. \cite{GaZa17}, Smirnov et al. \cite{SmGl17}, Pozo et al. \cite{PoRo18}, Jin et al. \cite{JiXi19}, Wang et al. \cite{WaCh20}, Reusch et al. \cite{ReZh20}, Yan et al. \cite{YaQu20}, Reusch et al. \cite{RePo20}, Houtan et al. \cite{HoAs21}, Syed et al. \cite{SyAy20} \\\hline
    \end{tabular}
    \caption{Categorization of research work based on optimization objective. }
    \label{tab:objectives}
\end{table}



==> chapters/05_features.tex <==
\section{Features}
\label{sec:features}
The following section gives an overview of research domains found in the literature. 
To give a comprehensive overview of which research work covers which domain, we compiled the classification in Table \ref{tab:features}.
% @TODO Introductory words, what is covered by the section

\begin{table*}[ht]
    \centering
    \begin{tabular}{|M{2.8cm}|M{1cm}|M{1cm}|M{1.8cm}|M{1cm}|M{1.6cm}|M{2cm}|M{1.2cm}|M{1.3cm}|}
    \hline
        Research work & \ac{AVB} & \ac{BE} & Joint Routing & Queuing & Fixed \ac{GCL} length & Reconfiguration & Reliability & Multicast \\\hline\hline
    Duerr et al. \cite{DuNa16}  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Pop et al. \cite{PoRa16}  & \cmark & \xmark & \xmark & (\cmark) & \xmark & \xmark & \xmark & Only \ac{AVB} \\\hline
    Craciunas et al. \cite{CrOl16}  & \xmark& \xmark  & \xmark & (\cmark) & \xmark & \xmark & \xmark & \xmark \\\hline
    Farzaneh et al. \cite{FaKu17}  & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  & \xmark \\\hline
    Gavrilut et al. \cite{GaZa17}  & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark \\\hline
    Raagaard et al. \cite{RaPo17}  & \xmark & \xmark & \xmark & (\cmark) & \xmark & \cmark & \xmark & \xmark \\\hline
    Schweissguth et al. \cite{ScDa17}  & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Smirnov et al. \cite{SmGl17}  & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark \\\hline
    Steiner et al. \cite{StCr18}  & \xmark & (\cmark) & \xmark & (\cmark) & \cmark & \xmark & \xmark & \cmark \\\hline
    Falk et al. \cite{FaDu18}  & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Gavrilut et al. \cite{GaPo18}  & \cmark & \xmark & \xmark & (\cmark) & \xmark & \xmark & \xmark & \xmark\\\hline
    Oliver et al. \cite{OlCr18}  & \xmark & (\cmark) & \xmark & (\cmark) & \cmark & \xmark &  \xmark & \cmark \\\hline
    Gavrilut et al. \cite{GaZh18}  & \cmark & \xmark & \cmark & (\cmark) & \xmark & \xmark &  \xmark & \xmark \\\hline
    Pozo et al. \cite{PoRo18}  & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark &  \cmark & \cmark \\\hline
    Pahlevan et al. \cite{PaOb18}  & \xmark &  (\cmark) & \cmark & (\cmark) & \xmark & \xmark & \xmark & \xmark \\\hline
    Pahlevan et al. \cite{PaTa19}  & \xmark &  (\cmark) & \cmark & (\cmark) & \xmark & \xmark & \xmark & \xmark \\\hline
    Jin et al. \cite{JiXi19} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Alnajim et al. \cite{AlSa19} & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Atallah et al. \cite{AtBa20} & \xmark & \xmark & \cmark & (\cmark) & \xmark & \xmark & \cmark & \xmark \\\hline
    Hellmanns et al. \cite{HeGl20}  & \xmark &  (\cmark) & \xmark & (\cmark) & \xmark & \xmark & \xmark  & \xmark \\\hline
    Falk et al. \cite{FaDu20}  & \xmark &  \xmark & \cmark & \xmark & \xmark & \xmark & \xmark  & \xmark \\\hline
    Jin et al. \cite{JiXi20}  & \xmark & (\cmark) & \xmark & (\cmark) & \cmark & \xmark & \xmark & \xmark \\\hline
    Reusch et al. \cite{ReZh20}  & \xmark & (\cmark) & \xmark & \cmark & \cmark & \xmark & \xmark  & \xmark \\\hline
    Wang et al. \cite{WaCh20}  & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark  & \xmark\\\hline
    Yan et al. \cite{YaQu20}  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark  & \xmark \\\hline
    Syed et al. \cite{SyAy20} & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark\\\hline
    Reusch et al. \cite{RePo20} & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark \\\hline
    Li et al. \cite{LiLi20} & \xmark & & \cmark & \xmark & \xmark & \xmark & \xmark \\\hline
    Houtan et al. \cite{HoAs21}  & \xmark & \cmark & \xmark & (\cmark) & \xmark & \xmark & \xmark & \xmark \\\hline
    Syed et al. \cite{SyAy21}  & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark\\\hline
    Zhou et al. \cite{ZhSa21} & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark \\\hline
    Mahfouzi et al. \cite{MaAm21} & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\\hline
    
    \end{tabular}
    \caption{Overview of additional features of scheduling algorithms in the literature. Indirect handling of \ac{BE} traffic and queuing with flow or frame isolation constraints is denoted by (\cmark). }
    \label{tab:features}
\end{table*}

\subsection{Joint Handling of \ac{AVB} Traffic}
Most studies in the field of \ac{TSN} scheduling have not dealt with \ac{AVB} traffic. 
Although most research works note that \ac{AVB} traffic exists beside \ac{TT} traffic, only two propose a joint handling approach for \ac{TT} and \ac{AVB} flows. 
Pop et al. \cite{PoRa16} present a \ac{GRASP} heuristic to deal with \ac{AVB} traffic.
Their heuristic computes a routing for \ac{AVB} flows, such that they meet their deadlines.
It reduces the search space by only considering a fixed number of shortest paths for every pair of nodes as possible routings. 
The schedule of \ac{TT} flows, computed by their \ac{ILP} model, serves as input parameter for the heuristic and cannot be changed.
They compare their \ac{AVB} routing with the naive approach of always selecting the shortest path.
The comparison shows that more flows can be scheduled with their approach. 
Gavrilut et al. \cite{GaPo18} also propose the use of a \ac{GRASP} heuristic for scheduling \ac{TT} flows while taking \ac{AVB} traffic into account.
In contrast to \cite{PoRa16}, their approach handles \ac{TT} and \ac{AVB} flows simultaneously. 
The routing of \ac{AVB} flows cannot be changed, so the only degree of freedom which affects \ac{AVB} flows is the scheduling of \ac{TT} flows.
Their evaluations show that using the \ac{GRASP} heuristic with an objective that considers tardiness of \ac{AVB} flows leads to schedules where \ac{AVB} flows meet their deadlines, in contrast to the \ac{GRASP} heuristic with other objectives.
Indeed, it is not a surprise that not taking \ac{AVB} flows into account leads to schedules with late \ac{AVB} flows.
In later works, Gavrilut et al. \cite{GaZh18} refined the \ac{GRASP} heuristic from \cite{GaPo18} for scheduling of \ac{TT} and \ac{AVB} flows.
Instead of a fixed routing, they suggest a routing heuristic which uses k-shortest paths.
They only route \ac{TT} flows, but note that routing of \ac{AVB} flows is only omitted for the sake of simplicity.
Their heuristic considers a schedule as infeasible if a \ac{TT} flow misses his deadline, and use minimization of the tardiness of \ac{AVB} flows as objective. 
In their evaluations, they were able to construct test cases where all \ac{AVB} flows can be scheduled when routing of \ac{TT} flows is considered before scheduling, but not otherwise.

\subsection{Considerations for \ac{BE} Traffic}
\ac{BE} traffic has no strict deadline requirements and may arise unpredictably.
Therefore, scheduling algorithms for \ac{TT} flows can only try to increase the \ac{QoS} of \ac{BE} traffic. 
As the use of guard bands or preemption reduce the time available for \ac{BE} traffic, reducing the number of gate-events benefits this traffic class.
Such an attempt is pursued by Jin et al. \cite{JiXi20}, with the objective of minimizing the number of \ac{GCL} entries.
The authors of \cite{StCr18}, \cite{OlCr18}, and \cite{ReZh20} schedule flows to a fixed number of transmission windows per egress port, also effectively limiting the number of gate-events and thus the number of guard bands. 
Another approach is the reduction of the flowspan, such that more continuous time is available to lower priority traffic exclusively.
Reducing the flowspan may also benefit the number of gate-events, as unnecessary interrupts between frame transmissions may be reduced.
For this reason, scheduling algorithms with the objective of reducing the flowspan have an indirect influence on \ac{BE} traffic.
Such research work is presented by Pahlevan et al. \cite{PaOb18} \cite{PaTa19} and Hellmanns et al. \cite{HeGl20}.
Duerr et al. \cite{DuNa16} also minimize the flowspan, but additionally present a compression algorithm which reduces the number of gate-events.
They note that this increases the available time for \ac{BE} traffic by reducing the number of guard bands. 
Alnajim et al. \cite{AlSa19} compare multiple incremental scheduling algorithms in regard of the number of guard bands needed.
They also note that reducing the number of guard bands is beneficial to \ac{BE} traffic.
The authors of \cite{HoAs21} perform an analysis of the impact of different scheduling objectives to \ac{QoS} of \ac{BE} traffic. 
Their evaluations show that gaps between \ac{TT} flows increase the \ac{QoS} of \ac{BE} flows.
However, it is important to note that the used system model features deadlines for \ac{BE} traffic, and they measure the number of deadline misses, so a comparison with the other mentioned research work is not appropriate.

\subsection{Joint Routing}
The first research work that addresses joint scheduling and routing for \ac{TT} flows in \ac{TSN} is presented in \cite{GaZa17}.
The authors propose two heuristics and a \ac{CP} model to compute a routing such that all \ac{TT} flows meet their deadlines.
All three approaches also solve the problem of topology synthesis.
Their optimization objective captures worst-case end-to-end delays as well as topology cost.
Gavrilut et al. \cite{GaZh18} address joint routing and scheduling of \ac{TT} and \ac{AVB} flows in their approach. 
They propose a routing heuristic, which only considers the k-shortest paths between two nodes.
The flows are processed one after another, and the path with the lowest utilization so far is chosen.
The routing is used as input to the scheduling, so it is fixed at scheduling time.
Their evaluations show that this routing approach increases schedulability of \ac{TT} flows with their GRASP heuristic in the next step considerably. 
Other research work about joint routing assumes the topology as fixed. 
Falk et al. \cite{FaDu18} give an \ac{ILP} model for joint scheduling and routing.
As they do not use an objective function, they are only interested in finding some feasible schedule and routing. 
Another \ac{ILP} approach for joint routing and scheduling was independently developed by Schweissguth et al. \cite{ScDa17}.
Their objective is to minimize the flow latencies.
Their evaluations show that schedulability increases considerably compared to the same test cases with a fixed routing. 
The authors of \cite{SmGl17} propose a \ac{PBO} model for joint routing and scheduling.
Their results imply that solving routing and scheduling separated reduces the overall solving time.
They state that instances with more routing options lead to easier to solve scheduling problems, as flows get more distributed over the network.
In \cite{FaDu20}, Falk et al. present an algorithm for joint scheduling and routing, which is not based on transmission constraints of flows.
They construct a conflict graph, where every vertex corresponds to schedule and routing of a single flow.
This reduces the scheduling problem to finding an independent set in the conflict graph.
The authors of \cite{AtBa20} first present a \ac{GRASP} heuristic for routing, which considers some reliability constraints.
The resulting routing is used as input to an iterative \ac{ILP} approach, which schedules groups of flows one after another based on a conflict measure.
Like \cite{FaDu18}, they do not use an objective function and only try to find some feasible schedule and routing.
An \ac{ILP} model for joint routing and scheduling for an in-vehicle network is presented in \cite{SyAy20}.
They compute schedules and routing for static flows, such that as many flows as possible can be added dynamically.
The same authors present in later work \cite{SyAy21} heuristics to compute scheduling and routing of such dynamically added flows to an already existing scheduling of static flows.
Pahlevan et al. \cite{PaOb18} use a genetic algorithm for joint scheduling and routing. 
While their evaluations indicate that solving time increases compared to scheduling with a fixed routing, they show that schedulability increases by joint scheduling and routing. 
The authors of \cite{PaTa19} propose a heuristic list scheduling algorithm.
They compare it to the same heuristic used as comparison in \cite{PaOb18}.
Their evaluations again show that joint routing and scheduling increases schedulability.
Wang et al. \cite{WaCh20} present ant colony optimization and genetic algorithm approaches to the routing and schulding problem.
Unfortunately, they do not elaborate on the routing, and the only related evaluation shows that increasing the number of edges increases the solving time.
Separate \ac{CP} models for routing and scheduling are presented in \cite{RePo20}.
The routing computed with the first model is used as a fixed parameter for the second model, similar to \cite{AtBa20}.
Alnajin et al. \cite{AlSa19} present a \ac{QoS}-aware routing algorithm for \ac{TSN} flows with respect to various metrics.
They evaluate schedulability with various scheduling algorithms combined with these routings.
Zhou et al. \cite{ZhSa21} propse the only \ac{SMT} model for joint scheduling and routing. 
Similar to \cite{AtBa20}, an iterative scheme is used.
Subsets of flows are scheduled and routed one after another until all flows are processed.
The schedules and flows of an iteration are fixed for subsequent iterations.
Another iterative scheme for scheduling and routing is presented by Mahfouzi et al. \cite{MaAm21}. 
Instead of grouping flows by some conflict measure, they split the network period in slices and group them by the time slice they start.
They allow routing only over some fixed number of precomputed shortest paths per source-destination pair, similar to \cite{GaZh18} and the \ac{AVB} routing in \cite{PoRa16}.
Their evaluations show a huge impact to solving time of the number of allowed paths, but they also note that schedulability is already over 90\% for three or more paths.
They conclude that the search space can be considerably reduced with negligible impact on schedulability. 
A special case for joint routing is considered in \cite{PoRo18}.
After a link failure, all flows over this link must be rescheduled and rerouted.
The authors propose a repair algorithm for this purpose.

\subsection{Queuing}
Most research work so far employs temporal or spatial isolation of different flows or frames of different flows.
The rational of this is the observation, that interleaved frames of different flows, which are at the same time in the same queue, may lead to non-deterministic behavior. 
This may be the case in the presence of other non-deterministic behavior, e.g. packet loss or synchronization errors. 
Reasoning and in-depth analysis of this matter is presented in \cite{CrOl16}.
Most later work references to this reasoning.
The authors compare the impact of frame and flow isolation to the solving time of a \ac{SMT} model.
Besides isolation in the time domain, they also employ isolation in the spatial domain by the possibility of assigning different flows to different queues. 
Their evaluations show that flow isolation can reduce solving time compared to frame isolation.
However, schedulability increases for frame isolation.
The authors were able to construct problem instances which are schedulable with frame isolation, but not with flow isolation.
The frame isolation constraint from \cite{CrOl16} is reused in \cite{PoRa16} and \cite{GaZh18}, but queuing is not the emphasis of these works.
Raagaard et al. \cite{RaPo17} restrict schedules to comply with flow isolation.
When a new flow should be added to an existing schedule, they calculate whether there is a starting offset such that the flow can be scheduled.
If this is not possible, the flow is successively assigned to new queues of the egress ports along its path.  
The window-based \ac{SMT} model of \cite{StCr18} and \cite{OlCr18} also use flow isolation to restrict the problems of non-deterministic behavior.
Two queues per egress port are dedicated for \ac{TT} traffic in this approach, so the number of \ac{TT} queues per port is fixed.
Gavrilut et al. \cite{GaPo18} report that \ac{AVB} traffic does not benefit from minimizing the number of queues for \ac{TT} flows.
However, their system model assumes \ac{AVB} flows already have an assignment to \ac{AVB} queues, so \ac{AVB} traffic cannot benefit from a lower number of \ac{TT} queues. 
The heuristics of Pahlevan et al. presented in \cite{PaOb18} and \cite{PaTa19} employ flow isolation to prevent interleaving of frames of different flows.
In contrast to \cite{GaPo18}, \cite{CrOl16}, \cite{OlCr18}, and others, only a single queue per egress port is dedicated to \ac{TT} traffic.
Another approach with only one queue for \ac{TT} traffic per egress port, but frame isolation in the temporal domain, is shown in \cite{AtBa20}.
The authors state that frame isolation eliminates the randomness of queuing delay. 
Houtan et al. \cite{HoAs21} show how frame and flow isolation can be integrated in their \ac{SMT} model. 
Unfortunately, their work lacks evaluations regarding the difference of both approaches or a description which was used in the evaluations.
As flow isolation implies frame isolation, integrating both simultaneously is not reasonable. 
Hellmanns et al. \cite{HeGl20} use the Tabu Search algorithm of \cite{DuNa16} for no-wait scheduling of flows in a ring network, so no queuing is needed.
However, they employ queues as buffer memory for flows with a destination in another ring network. 
When all flows between nodes in the same ring have finished, the gates of the buffer queues are opened and the remaining schedule is computed by a simulation. 
The approach of \cite{JiXi20} is even more restrictive than frame isolation, as only exactly one packet is allowed in a queue at any given time. 
Their approach allows multiple queues for \ac{TT} traffic per egress port, but assigning flows to queues is not part of the \ac{SMT} model.
Assigning flows to queues is done before solving the \ac{SMT} model by a greedy heuristic, which aims to balance the workload of all queues of an egress port.
Both isolation constraints are dropped in \cite{ReZh20}.
A worst-case delay analysis using Network Calculus is employed instead to provide real-time guarantees of computed schedules.
Alnajim et al. \cite{AlSa19} also allow a bounded queuing delay in one of the presented algorithms.
Their evaluations show that schedulability increases and the number of guard bands can be reduced considerably by allowing queuing.
Mahfouzi et al. \cite{MaAm21} present a \ac{SMT} model for joint routing and scheduling which allows queuing, but do not evaluate anything queuing related.
Yan et al. \cite{YaQu20}

\subsection{Fixed \ac{GCL} Length}
Most past work has not considered the fact, that \acp{GCL} in real bridges only have a limited number of entries. 
\acp{GCL} are synthesized via post-processing from a schedule.
Notable exceptions include \cite{ReZh20}, \cite{StCr18}, and \cite{OlCr18}.
The respective authors propose window-based \ac{SMT} models.
Only a fixed number of transmission windows is integrated at generation time of the model.
They tread the scheduling of frames as the problem of assigning frames to windows of an egress port.
With a fixed number of windows per egress port, there is also a fixed number of gate-open and gate-close events per egress port.
Jin et al. \cite{JiXi20} present research work dedicated to the problem of a limited number of \ac{GCL} entries.
They propose a \ac{SMT} model with an explicit coding of gate-events.
An iterative scheme is used for performance reasons, where subsets of flows are schedules one after another.
The objective when optimizing a subset is to minimize the maximal number of \ac{GCL} entries for all egress ports.
They also give a heuristic algorithm which complies with a limited number of \ac{GCL} entries.
The number of needed entries, solving time, and schedulability are compared. 
Their evaluations show that the heuristic algorithm is an order of magnitude faster than naive algorithms from the literature, while reducing the number of \ac{GCL} entries considerably. 

\subsection{Reconfiguration}
Little work has been done about dynamic reconfiguration. 
Syed et al. \cite{SyAy20} present some preliminary work about scheduling and routing for in-vehicle networks, which are computed offline for static flows and are suitable for adding dynamic flows.
In later work \cite{SyAy21}, the same authors give multiple heuristics for dynamic reconfiguration of scheduling and routing.
They evaluate the solving time needed for adding varying numbers of flows, as reconfiguration in a car has strict time requirements.  
The authors of \cite{RaPo17} propose a heuristic to reconfigure the scheduling when new flows are added, though they don't handle routing.
Their approach assigns new flows to other queues if adding the flow would invalidate the schedule otherwise.

\subsection{Reliability Considerations}
Most research work which concerns reliability utilizes redundant flows routed through link-disjoint paths. 
So, all of them also feature joint routing.
The authors of \cite{AtBa20} replicate flows to comply with requirements regarding robustness to link failures.
Computed schedules are only valid if redundant copies of a flow have disjoint paths. 
The same approach is pursued by Reusch et al. \cite{RePo20}.
In contrast to \cite{AtBa20} and \cite{RePo20}, the authors of \cite{GaZa17} can also alter the topology to fulfill such requirements.
Repairing of schedules for \ac{TT} traffic is considered in \cite{PoRo18}.
The authors propose a fast heuristic to reroute and reschedule frames affected by a link failure. 
They also evaluate which properties of a schedule are beneficial for repairability. 
The results indicate that schedules which maximize the distance between frames are much easier to repair than schedules which minimize the flowspan, even for three simultaneous link failures.
Instead of tolerance for link failures, Zhou et al. \cite{ZhSa21} consider reliability for transient loss.
They integrate constraints regarding reliability along the routed path of a flow in their \ac{SMT} model.
However, the reliabilities of paths are only approximated, as the used theory solver can not handle exponentials. 
They also use redundant copies of flows to further decrease the probability of transient loss, as there may be no single path with the required reliability, but do not enforce the paths to be link disjoint like \cite{AtBa20}, \cite{RePo20}, and \cite{GaZa17}.
Their evaluations show that schedulability with a given level of reliability against transient faults increases with an increased number of redundant copies.

\subsection{Multicast}
Most research work does not handle multicast explicitly. 
Some papers state that multicast is a trivial extension, as a multicast flow can be expressed as multiple unicast flows.
However, this would inflate the resulting models and problem instances, so we only consider research work with explicit handling of multicast flows here.
Gavrilut et al. \cite{GaZa17} regard multicast flows in their topology synthesizes and routing problem. 
As they include redundant copies of flows in their model to increase fault-tolerance, multicast trees must be link disjoint. 
Smirnov et al. \cite{SmGl17} state that multicast flows can be expressed by unicast flows, but also describe how these unicast flows can efficiently be modelled without the overhead of shared links. 
Steiner et al. \cite{StCr18} allow multicast flows in their model, although they do not elaborate on this matter.
However, a technical report by the same authors which details on the model indicates that they use the same approach as \cite{SmGl17}.
Pahlevan et al. \cite{PaOb18} \cite{PaTa19} state multicast capabilities as one of their main contributions, but consider multicast flows as multiple unicast flows, too.
Pozo et al. \cite{PoRo18} present an ILP in which construction does not depend on whether flows are unicast or multicast. 
They evaluate the impact of a higher percentage of broadcast and multicast flows on the solving time of their ILP.

==> chapters/06_evaluations.tex <==
\section{Evaluations}
\label{sec:evaluations}
In the following section, we dive more into the details of the reported evaluations and their results. 
First, we introduce the used problem instances in the literature.
Then, we present results regarding scalability of the presented algorithms and schedulability in the respective scenarios.
We conclude the section with an overview of other interesting evaluations and insights from the research body of TSN scheduling.

\subsection{Problem Instances}
Before we describe evaluation results, we will have a look at the problem instances used.
Unfortunately, some research work does not elaborate on the used topologies, which makes assessing and comparing the results to other works harder. 
Most research work handles only synthetic test cases. 
The most common topologies encountered are ring graphs  \cite{FaDu18}\cite{FaDu20}\cite{HeGl20}\cite{YaQu20}\cite{PaOb18}\cite{PaTa19}.
Hellmanns \textit{et al.} \cite{HeGl20} argue that rings are a common topology in real-world industrial facilities.
Other systematic topologies used include line \cite{FaDu18}\cite{OlCr18}\cite{YaQu20}, grid  \cite{PaOb18}\cite{PaTa19}, and snowflake-like \cite{FaKu17}\cite{GaPo18}\cite{ReZh20}\cite{YaQu20}\cite{HoAs21} graphs. 
Various randomized topologies are also used for evaluation.
Erdős–Rényi graphs are the most common one \cite{DuNa16}\cite{FaDu18}\cite{ZhSa21}, but Barabási-Albert graphs \cite{DuNa16}\cite{FaDu18} and random regular graphs  \cite{DuNa16} are also used.
There is also a small number of  research work concerned with real-world topologies. 
Syed \textit{et al.} \cite{SyAy20}\cite{SyAy21} use  a real-world car architecture for their evaluations. 
Zhou \textit{et al.} \cite{ZhSa21} conclude their evaluations by investigating a real-world example from General Motors. 
The authors of \cite{GaZa17} also use a real-world use case from General Motors.
However, as topology generation is part of their problem, this instance is rather a set of flows. 
All research work concerned with synthetic test cases uses randomly generated flows.
Source and destination of these flows were chosen uniformly from the set of nodes in the network.
The number of flows varies considerably between different research works.  
It ranges from 2 flows in the smallest instance in Falk \textit{et al.} \cite{FaDu18} to up to 10000 flows in the largest instance of Jin \textit{et al.} \cite{JiXi19}.

Table \ref{tab:instances} compiles the most important information about the problem instances used for evaluations.
% TODO Eileitender Text für subsection schreiben
\begin{table}[ht]
    \centering
    \begin{tabular}{|M{2.3cm}|M{1.3cm}|M{0.9cm}|M{0.9cm}|M{1.2cm}|}
    \hline
     Research work & Topology & ES & Bridges & Flows \\\hline\hline
    Duerr \textit{et al.} \cite{DuNa16}  & ER, RRG, BA & 24--100 & 5--20 & 30--1500  \\\hline
    Pop \textit{et al.} \cite{PoRa16}  & N/A & 3--5 & 1--2 & 3--5 \\\hline
    Craciunas \textit{et al.} \cite{CrOl16}  & N/A & 3--7 & 1--5 & 5--1000 \\\hline
    Farzaneh \textit{et al.} \cite{FaKu17}  & Snowflake & 12 & 2 & 14--100 \\\hline
    Gavrilut \textit{et al.} \cite{GaZa17}  & N/A & 4--20 & N/A & 4--38  \\\hline
    Raagaard \textit{et al.} \cite{RaPo17}  & N/A & \multicolumn{2}{c|}{4--402} & 15--290 \\\hline
    Schweissguth \textit{et al.} \cite{ScDa17}  & Ring, Partial mesh & 12 & 12  & 20--52 \\\hline
    Steiner \textit{et al.} \cite{StCr18}  & N/A & 50 & 10 & 10--50  \\\hline
    Falk \textit{et al.} \cite{FaDu18}  & Line, Ring, BA, ER & \multicolumn{2}{c|}{5--36} & 2--30\\\hline
    Gavrilut \textit{et al.} \cite{GaPo18}  & Star, Snowflake & 3--32 & 1--18 & 4--35 \\\hline
    Oliver \textit{et al.} \cite{OlCr18}  & Line & 50 & 10 & 10--50 \\\hline
    Pozo \textit{et al.} \cite{PoRo18}  & Synthetic & 6--8 & 3--8 & 10--50 \\\hline
    Pahlevan \textit{et al.} \cite{PaOb18}  & Grid, Ring & 27--45 & 9 & 30--40  \\\hline
    Pahlevan \textit{et al.} \cite{PaTa19}  & Grid, Ring & 50 & 10 & 60--100 \\\hline
    Jin \textit{et al.} \cite{JiXi19} & N/A & 5--30 & 5--30 & 10--60 \\\hline
    Alnajim \textit{et al.} \cite{AlSa19} & N/A & 30--150 & 10--50 & 100--1500\\\hline
    Atallah \textit{et al.} \cite{AtBa20} & N/A & N/A & 3--21 & 20--60   \\\hline
    Hellmanns \textit{et al.} \cite{HeGl20}  & Ring of rings & \multicolumn{2}{c|}{100--2500} & 10--2000 \\\hline
    Falk \textit{et al.} \cite{FaDu20} & Ring w/ $k$ neighbors & \multicolumn{2}{c|}{50--400} & 50--150 \\\hline
    Jin \textit{et al.} \cite{JiXi20}  & N/A & N/A & 6--20 & 10--10000 \\\hline
    Reusch \textit{et al.} \cite{ReZh20}  & Snowflake & 3--256 & 1--146 & 14--316 \\\hline
    Wang \textit{et al.} \cite{WaCh20}  & N/A & 25 & 5 & 10--100 \\\hline
    Yan \textit{et al.} \cite{YaQu20}  & Line, Ring, Snowflake & \multicolumn{2}{c|}{15} & 500--2000  \\\hline
    Syed \textit{et al.} \cite{SyAy20} & Real-world car & N/A & N/A & 20--90 \\\hline
    Reusch \textit{et al.} \cite{RePo20} & Various & 4--32 & 1--16 & N/A \\\hline
    Houtan \textit{et al.} \cite{HoAs21}  & Snowflake & 6 & 2 & 10 \\\hline
    Syed \textit{et al.} \cite{SyAy21}  & Real-world car & N/A & N/A & 100--500 \\\hline
    Zhou \textit{et al.} \cite{ZhSa21} & ER, Real-world & 16 & 6--10 & 50--380\\\hline
    \end{tabular}
    \caption{Overview of inspected instances in the literature, sorted by publication year.}
    \label{tab:instances}
\end{table}

\subsection{Scalability}
Almost all research work about TSN scheduling includes or even focuses on evaluations about the scalability of the proposed approach. 
Most of these evaluations measure the solving time of selected instances.
We identified two tendencies in regard to solving time of the algorithms from the literature:
First, heuristic algorithms can handle larger instances than approaches with exact solution methods.
Second, exact algorithms which perform joint routing and scheduling can only handle smaller instances compared to algorithms solely for scheduling. 
Table \ref{tab:runtime} compiles the reported runtimes for the largest instance that could be solved in the respective research work.
It is meant to show general tendencies and improvements over time.
Caution is needed when interpreting the table, as it shows the reported times after which an  algorithm terminated, not the time until a first valid schedule could be obtained, as almost all papers do not report this time, not to  suggest one  approach over the other. 
This is a systematic disadvantage of exact approaches, as they only terminate when the optimal solution is found or a timeout is reached, while heuristic algorithms terminate much earlier with suboptimal results.
Some research work deals with more parameters than the size of the network and the number of flows, e.g. \cite{OlCr18} with the number of transmission windows per egress port, or handles additional problems simultaneously, like joint routing or AVB scheduling. 
Approximations are given when results are not stated in the text and had to be estimated by the presented figures. 
Ranges are given when multiple instances are considered to be the largest.
The following sections will report results regarding scalability, divided by solution approach.

\subsubsection{Exact Approaches}
The evaluations of Falk \textit{et al.} \cite{FaDu18} show that solving time is more influenced by the number of flows than the size of the network for their ILP. 
They also show that the network topology has an impact on scalability. 
Network topologies with more paths between any pair of nodes tend to yield easier problem instances, as less flows compete for the same links.
The higher the occupation of the links from transmissions, the harder to solve is a problem instance.
Pop \textit{et al.} \cite{PoRa16} compare their ILP to the SMT from \cite{CrOl16}, which is inconclusive. 
They state that their proposed ILP does not scale well for industrial size instances.
Schweissguth \textit{et al.} \cite{ScDa17} compare the solving time of their ILP for joint routing and scheduling with ILPs solely for scheduling.
As expected, solving time increases for joint routing and scheduling.
Nevertheless, they still recommend joint routing, as solution quality increases considerably.
Smirnov \textit{et al.} \cite{SmGl17} compare a PB approach for joint routing and scheduling with the corresponding 2-step approach.
Surprisingly, their evaluations show that the 2-step approach performs significantly worse for larger instances.
They explain this behavior by the capability of SAT solvers to learn from conflicts, which is lost after the routing step.
Atallah \textit{et al.} \cite{AtBa20} compare their ILP for joint routing and scheduling with the ILPs from \cite{SmGl17} and \cite{ScDa17}. 
It outperforms both in regard to solving time in their evaluations.
In \cite{CrOl16}, the authors investigate the scalability of their SMT approach in regard to the use of frame isolation and flow isolation.
Their evaluations show that flow isolation always yields models which can be solved faster.
The authors of \cite{OlCr18} evaluate the solving time of their SMT approach with respect to the number of flows and the number of transmission windows per port.
Their results show that the solving times grows exponentially for the number of flows, while it grows polynomial for the number of transmission windows.
However, for reasonable numbers of flows and  transmission windows, solving time is more sensible to  the number of transmission windows.
A comparison to the SMT from \cite{CrOl16} shows that their window-based approach with one window per egress port outperforms their older approach.
Farzaneh \textit{et al.} \cite{FaKu17} observe that solving time increases when the size of the flows increases or when flows of different periods are part of an  instance.
The state that the solving time is reasonable for up to 100 flows, where solving time begins to grow exponentially.
The authors of \cite{HoAs21} show that solving time for their SMT depends heavily on the objective function used.
Jin \textit{et al.}  \cite{JiXi19} show that the instance size  which can be solved by their  SMT  approach is limited.
Their proposed heuristic algorithms can schedule instances an order of magnitude larger.
The same holds for \cite{JiXi20}, where instances with up to 10000 flows could be scheduled in reasonable time,  while the SMT approach could not produce a feasible schedule for an instance with 100 flows within 2 days.
Pozo \textit{et al.} \cite{PoRo18} evaluate the impact of the traffic type distribution to solving time. 
They observe that solving  time increases with more multicast and broadcast flows, as the generated ILP gets more variables.


\subsubsection{Heuristic Approaches}
Duerr \textit{et al.} \cite{DuNa16} measure the solving times of their Tabu Search and conclude, that the network topology and size have no impact on solving time.
However, they only compare random network topologies which contain many links and thus many paths.
Gavrilut et  al. \cite{GaPo18} show that solving time of their GRASP  heuristic increases considerably when AVB flows are taken into account.
The authors of \cite{GaZa17} compare their CP approach with a GRASP heuristic to compute routing, schedule, and topology. 
As expected, the CP approach does not scale well and the GRASP heuristic finds better solutions in minutes compared to the CP approach in two days.
Hellmanns \textit{et al.} \cite{HeGl20} employ the Tabu Search from \cite{DuNa16} in a 2-step approach for ring networks which are interconnected by a ring.
They compare this approach with scheduling the whole network at once.
Their evaluations show that there approach scales better for networks with many flows, as the original approach does not produce results for more than 1000 flows due to memory limitations. 
The 2-stage approach is more than two orders of magnitude faster for this special case.
Raagaard \textit{et al.} \cite{RaPo17} present a heuristic for dynamic rescheduling, which is able to schedule about 1300 frames per second in the presented test cases. 

\begin{table}[ht]
    \centering
    \begin{tabular}{|M{2.3cm}|M{1.3cm}|M{0.75cm}|M{0.75cm}|M{1.4cm}|}
    \hline
    Research work & Solution Approach & Nodes & Flows & Runtime (s) \\\hline\hline
    \multicolumn{5}{|c|}{Exact Approaches w/o Joint Routing} \\\hline
    Pop \textit{et al.} \cite{PoRa16}  & ILP & 7 & 5 & $80.19$ \\\hline
    Craciunas \textit{et al.} \cite{CrOl16}  & SMT & 12 & 1000 & $< 18000$ \\\hline
    Farzaneh \textit{et al.} \cite{FaKu17}  & SMT & 14 & 100 & $< 240$ \\\hline
    Oliver \textit{et al.} \cite{OlCr18}  & SMT & 20 & 750 & $\sim 600$ \\\hline
    Steiner \textit{et al.} \cite{StCr18}  & SMT & 60 & 50 & $\sim 0.01$ -- $100$ \\\hline
    Jin \textit{et al.} \cite{JiXi19}  & SMT & 4 & 4 & $< 600$ \\\hline
    Jin \textit{et al.} \cite{JiXi20}  & SMT & 6 & 50 & $660$--$1080$ \\\hline
    Houtan \textit{et al.} \cite{HoAs21}  & SMT & 8 & 10 & $0.37$--$1153.52$ \\\hline
    \multicolumn{5}{|c|}{Heuristic Approaches w/o Joint Routing} \\\hline
    Duerr \textit{et al.} \cite{DuNa16}  & Tabu Search & 120 & 1500 & 11520 \\\hline
    Gavrilut \textit{et al.} \cite{GaPo18}  & GRASP & 50 & 35 & $612.8$ \\\hline
    Jin \textit{et al.} \cite{JiXi20} & Heuristic & 20 & 10000 & $\sim 5100$ \\\hline
    Hellmanns \textit{et al.} \cite{HeGl20} & Tabu Search & 2500 & 2000 & $\sim 4400$ \\\hline
    Yan \textit{et al.} \cite{YaQu20}  & Heuristic & 15 & 2000 & $\sim 900$ \\\hline
    Raagaard \textit{et al.} \cite{RaPo17}  & Heuristic & 402 & 290 & 20--54 \\\hline
    Reusch \textit{et al.} \cite{ReZh20} & Heuristic & 402 & 316 & $10.52$ \\\hline
    \multicolumn{5}{|c|}{Exact Approaches w/ Joint Routing} \\\hline
    Gavrilut \textit{et al.} \cite{GaZa17} & CP & 20 & 38 & $172800$ \\\hline
    Schweissguth \textit{et al.} \cite{ScDa17}  & ILP & 24 & 52  & $1284.53$ \\\hline
    Falk \textit{et al.} \cite{FaDu18} & ILP & 8 & 30 & $\sim 170$ -- $1580$ \\\hline
    Pozo \textit{et al.} \cite{PoRo18}  & ILP & 16 & 50  & 2--85 \\\hline
    Atallah \textit{et al.} \cite{AtBa20} & ILP & 14 & 60 & $\sim 100$ \\\hline
    Syed \textit{et al.} \cite{SyAy20} & ILP & N/A & 90 & $\sim 21000$ \\\hline
    Reusch \textit{et al.} \cite{RePo20}  & CP & 48 & N/A & $\sim 1800$ \\\hline
    Zhou \textit{et al.} \cite{ZhSa21}  & SMT & 10 & 380 & $\sim 2700$ \\\hline
    \multicolumn{5}{|c|}{Heuristic Approaches w/ Joint Routing} \\\hline
    \multirow{2}{*}{Gavrilut \textit{et al.} \cite{GaZa17}}  & GRASP & 20 & 38 & $558$ \\\cline{2-5}
     & Heuristic & 20 & 38 & $130$ \\\hline
    \multirow{3}{*}{Pahlevan \textit{et al.} \cite{PaOb18}} & List scheduler & 45 & 40 & $0.014$ \\\cline{2-5}
     & Genetic algorithm & 45 & 40 & $56.75$ \\\hline
    \multirow{2}{*}{Pahlevan \textit{et al.} \cite{PaTa19}}  & List scheduler & 50 & 100 & $0.103$ \\\cline{2-5}
      & Heuristic & 50 & 100 & $1.58$ \\\hline
    Alnajim \textit{et al.} \cite{AlSa19} & Heuristic & 200 & 1500 & $2718$ \\\hline
    Falk \textit{et al.} \cite{FaDu20} & Heuristic & 400 & 400 & $\sim 6000$ -- $11000$ \\\hline
    Wang \textit{et al.} \cite{WaCh20}  & Heuristic & 30 & 100 & $72$ \\\hline
    Syed \textit{et al.} \cite{SyAy21}  & Heuristic & N/A & 500 & $0.170$ \\\hline
    \end{tabular}
    \caption{Overview of solution times of the respective largest reported problem instance for which a schedule could be found. We consider the instance with the highest number of flows as the largest instance. }
    \label{tab:runtime}
\end{table}

\subsection{Further Evaluation Results}
Dürr \textit{et al.} \cite{DuNa16} propose a compression algorithm for GCLs in addition to their scheduling ILP. 
They report that the number of GCL entries can be reduced by 24\% on average.
In subsequent works, the authors of \cite{HeGl20} show that the number of GCL entries is remarkably reduced by their 2-step approach.
Jin \textit{et al.} \cite{JiXi20} compare different algorithms which comply with a limited number of GCL entries.  
They propose to use a heuristic for fast construction of schedules and using an iterative OMT approach to reduce the number of GCL entries thereafter.
Alnajim \textit{et al.}  \cite{AlSa19} show that their heuristics can reduce the number of guard bands significantly in comparison to approaches with isolation constraints.
The authors of \cite{OlCr18} and \cite{StCr18} show in their evaluations, that the average jitter of all flows can be reduced significantly by increasing the number of transmission windows per egress port.
Pozo \textit{et al.} \cite{PoRo18} show that time gaps between frames on a link help to recover faster on average from link failures.
The authors of  \cite{ZhSa21} present evaluations which indicate that redundant flow copies increase the schedulability with reliability constraints.
Various research works show that scheduling with joint routing increases the schedulability compared to separated steps, as conflicting flows can be rerouted while scheduling \cite{PaOb18} \cite{PaTa19} \cite{ScDa17} \cite{SmGl17}. 
The authors of \cite{JiXi19} show that  schedulability increases considerably by  up top 50\% when message fragmentation is also taken into account while scheduling.

==> chapters/07a_other_works.tex <==
\section{Non-Peer Reviewed Works Regarding TSN Scheduling}
\label{sec:otherworks}
In this section, we highlight some works about TSN scheduling which were not published in a peer reviewed journal or conference.
Numerous PhD thesis are centered around TSN scheduling. 
To the best of our knowledge, the first PhD thesis about TSN scheduling was presented by Nayak \cite{Na18}.
One of the main contributions of his thesis is also published in \cite{DuNa16}, which influenced many research works in this area.
He also discusses research work regarding the use of SDN to TSN, which is out of scope of this survey.
Barzegaran \cite{Ba21} examines in his PhD thesis optimization in fog computing platforms.
Parts of the presented research related to TSN were published in \cite{BaPo21}.
The thesis also contains submitted but unpublished work about TSN in fog computing platforms, which is thus not in scope of this survey.
Dos Santos \cite{Sa20} presents an extensive framework to compute TSN schedules with many features only seen individually in previous works.
An implementation is also available.
The research work \cite{SaCa19} gives a summary of the features and techniques used in his approach.
Zhou \cite{Zh22} investigates in his PhD thesis scheduling in safety-critical systems.
The contributions regarding TSN in this thesis are also published in \cite{ZhSa21}, \cite{ZhSa21b}, and \cite{ZhSa22}.
Bachelor and master theses are rarely published and often not publicly available. However, multiple such theses drew our attention and are worth being mentioned. 
Caddell \cite{Ca18} developed a SMT model, which is used as a baseline in the evaluations of \cite{VlHa21b}.
Haug \cite{Ha20} conducted tests about parameter tuning and pre-processing to increase scalability of ILP models for joint scheduling and routing.
Many ideas and results of this thesis were published in \cite{HeHa21}.
Bansal \cite{Ba18} constructed a divide-and-conquer scheduling algorithm for TSN.
So far, there is no published research work which presents such an algorithm.
